A parametrized set of explicit elements of $\Sha(E/\Q)[3]$

In this paper, we give explicit equations for homogeneous spaces corresponding to a rational isogeny of degree $3$. An explicit set of elliptic curves with elements of order $3$ in their Tate-Shafarevich group is constructed. Combining this gives explicit examples of plane cubics over $\Q$ that have a point everywhere locally, but not globally.

==> AAPackages.tex <==

%% Language and font encodings
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{comment}
\usepackage[usenames,dvipsnames]{xcolor} %color comments

\usepackage{mathpazo}
\usepackage[colorlinks, linkcolor=BlueViolet, urlcolor=BlueViolet, citecolor=BlueViolet]{hyperref}
%\usepackage{showkeys}
\usepackage{bm}
\usepackage{verbatim}
\usepackage[margin=1in]{geometry}
\usepackage{array,multirow}
\usepackage{graphicx}
\usepackage{tikz-cd}
\usepackage{colonequals}
%\usepackage{tikz}
%\usetikzlibrary{positioning}
\usepackage{adjustbox}
\usepackage{booktabs}
\usepackage{comment}

\usepackage[all]{xy}
%\usepackage{tabu}
\usepackage{array}
\usepackage{tikz-cd}

\usepackage{caption}
\usepackage{subcaption}

\usepackage{amssymb,amsmath,latexsym,amsthm}%or any usual package
%\usepackage[main=english]{babel}
%\usepackage[cmtip,all]{xy}
\usepackage{multirow, cellspace}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}

\newtheorem*{theorem*}{Theorem A}
\newtheorem*{theorem'}{Theorem B}
\newtheorem*{theorem"}{Theorem C}

\newtheorem{problem}[theorem]{Problem}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{predefinition}[theorem]{Definition}
\newenvironment{definition}{\begin{predefinition}\rm}{\end{predefinition}}
\newtheorem{preremark}[theorem]{Remark}
\newenvironment{remark}{\begin{preremark}\rm}{\end{preremark}}
\newtheorem{prenotation}[theorem]{Notation}
\newenvironment{notation}{\begin{prenotation}\rm}{\end{prenotation}}
\newtheorem{preexample}[theorem]{Example}
\newenvironment{example}{\begin{preexample}\rm}{\end{preexample}}
\newtheorem{preclaim}[theorem]{Claim}
\newenvironment{claim}{\begin{preclaim}\rm}{\end{preclaim}}
\newtheorem{prequestion}[theorem]{Question}
\newenvironment{question}{\begin{prequestion}\rm}{\end{prequestion}}
\newtheorem{preapplication}[theorem]{Application}
\newenvironment{application}{\begin{preapplication}\rm}{\end{preapplication}}

%\theoremstyle{definition}
%\newtheorem{definition}{Definition}
%\newtheorem{remark}{Remark}
%\newtheorem*{example}{Example}
%\newtheorem*{application}{Application}
%\newtheorem*{question}{Question}


\newtheorem*{conjecture}{Conjecture}
\numberwithin{equation}{section}


%% Useful packages
\usepackage{amsfonts,amssymb,amsmath,amsthm,latexsym,dsfont}
\usepackage{pifont}% http://ctan.org/pkg/pifont
\usepackage{setspace}
\usepackage{mathtools}
\usepackage{epsfig}
\usepackage{amsfonts}
\usepackage{amsmath, amsthm, amssymb}
\usepackage{graphicx}
\usepackage{euscript}
%\usepackage[colorinlistoftodos]{todonotes}
\usepackage{enumerate}
\usepackage{tikz-cd}
\usepackage{listings}
\usepackage{pdfpages}
\usepackage{chngcntr}
\lstdefinelanguage{Magma}%
  {otherkeywords={:=,+:=,-:=,*:=},%
          % functions
   procnamekeys={function,func,intrinsic,procedure,proc},%
         % Booleans
   morekeywords={true,false},%
          % relations
   morekeywords=[2]{adj,and,cat,cmpeq,cmpne,diff,div,eq,ge,gt,in,is,join,le,lt,%
          meet,mod,ne,notadj,notin,notsubset,or,sdiff,subset,xor},%
          % keywords
   morekeywords=[3]{assigned,break,by,case,catch,continue,declare,default,%
          delete,do,elif,else,end,eval,exists,exit,for,forall,fprintf,if,local,%
          not,print,printf,quit,random,read,readi,repeat,restore,save,select,%
          then,time,to,try,until,vprint,vprintf,vtime,when,where,while},%
          % directives
   morekeywords=[4]{clear,forward,freeze,iload,import,load},%
          % error checks
   morekeywords=[5]{assert,assert2,assert3,error,require,requirege,requirerange},%
          % constructors
   morekeywords=[6]{car,comp,cop,elt,ext,frac,hom,ideal,iso,lideal,loc,map,%
          ncl,pmap,quo,rec,recformat,rep,rideal,sub},%
          % other constructors (semi-reserved)
   morekeywords=[7]{AbelianGroup,AdditiveCode,AffineAlgebra,Algebra,%
          AssociativeAlgebra,Character,CliffordAlgebra,Design,Digraph,%
          ExtensionField,FPAlgebra,FiniteAffinePlane,FiniteProjectivePlane,%
          Graph,Group,GroupAlgebra,IncidenceStructure,LieAlgebra,LinearCode,%
          LinearSpace,MatrixAlgebra,MatrixGroup,MatrixRing,Monoid,%
          MultiDigraph,MultiGraph,NearLinearSpace,Network,PartialMap,%
          PermutationGroup,PolycyclicGroup,QuaternionAlgebra,Semigroup,%
          ZModule},%
          % functions
   morekeywords={[8]function,func,intrinsic,procedure,proc,return},%
      sensitive,%
      morecomment=[l]//,%
      morecomment=[s]{/*}{*/},%
      morecomment=[s]{\{}{\}},%
      morestring=[b]"%
  }[keywords,procnames,comments,strings]%
\lstset{ 
  backgroundcolor=\color{white},   % choose the background color; you must add \usepackage{color} or \usepackage{xcolor}; should come as last argument
  basicstyle=\footnotesize,        % the size of the fonts that are used for the code
  breakatwhitespace=false,         % sets if automatic breaks should only happen at whitespace
  breaklines=true,                 % sets automatic line breaking
  captionpos=b,                    % sets the caption-position to bottom
  commentstyle=\color{black},    % comment style
  deletekeywords={...},            % if you want to delete keywords from the given language
  escapeinside={\%*}{*)},          % if you want to add LaTeX within your code
  extendedchars=true,              % lets you use non-ASCII characters; for 8-bits encodings only, does not work with UTF-8
  firstnumber=1,                % start line enumeration with line 1000
  frame=single,	                   % adds a frame around the code
  keepspaces=true,                 % keeps spaces in text, useful for keeping indentation of code (possibly needs columns=flexible)
  keywordstyle=\color{black},       % keyword style
  language=Magma,                 % the language of the code
  morekeywords={*,...},            % if you want to add more keywords to the set
  numbers=left,                    % where to put the line-numbers; possible values are (none, left, right)
  numbersep=5pt,                   % how far the line-numbers are from the code
  numberstyle=\tiny\color{black}, % the style that is used for the line-numbers
  rulecolor=\color{black},         % if not set, the frame-color may be changed on line-breaks within not-black text (e.g. comments (green here))
  showspaces=false,                % show spaces everywhere adding particular underscores; it overrides 'showstringspaces'
  showstringspaces=false,          % underline spaces within strings only
  showtabs=false,                  % show tabs within strings adding particular underscores
  stepnumber=1,                    % the step between two line-numbers. If it's 1, each line will be numbered
  stringstyle=\color{black},     % string literal style
  tabsize=2,	                   % sets default tabsize to 2 spaces
  title=\lstname                   % show the filename of files included with \lstinputlisting; also try caption instead of title
}
\numberwithin{equation}{section}
\numberwithin{figure}{section}
\numberwithin{table}{section}


\makeatletter
\def\keywords{\xdef\@thefnmark{}\@footnotetext}
\makeatother

%% Mathematical environments

%% Commands
\def \C {{\mathbb C}}
\def \E {{\mathbb E}}
\def \F {{\mathbb F}}
\def \L {{\mathbb L}}
\def \N {{\mathbb N}}
\def \P {{\mathbb P}}
\def \Q {{\mathbb Q}}
\def \R {{\mathbb R}}
\def \Z {{\mathbb Z}}
\def \O {{\mathcal O}}
\def \fp {{\mathfrak p}}
\def \fq {{\mathfral q}}
\def \a {\alpha}
\def \b {\beta} 
\def \g {\gamma}
\def \d {\delta}
\def \D {\Delta}
\def \x {\xi}
\def \y {\eta} 
\def \r {\rho}
\def \s {\sigma} 
\def \t {\tau}
\def \k {\kappa} 
\def \l {\lambda}
\def \th {\theta}
\def \om {\omega}
\def \Om {\Omega}
\def \ph {\varphi}
\def \mmu {\mathbf{\mu}}
\def \WNF {Weierstrass Normal Form\xspace}
\def \WCh {Weil-Ch\^{a}telet\xspace}
\def \phih {\hat{\phi}}
\def \psih {\hat{\psi}}
\def \chih {\hat{\chi}}
\def \Ktwo {K^\times/{K^\times}^2}
\def \Qtwo {\Q^\times/{\Q^\times}^2}
\def \Qthree {\Q^\times/{\Q^\times}^3}
\def \Lthree {L^\times/{L^\times}^3}
\def \Mm {M^\times/{M^\times}^m}
\def \Km {K^\times/{K^\times}^m}
\def \Lstar {L(S_{E,\psi},3)^*}
\def \Etors {E_{\textup{tors}}}
\def \tors {\textup{tors}}
\def \Gal{\textup{Gal}}
\def \WC{\textup{WC}}
\def \Cl {\textup{Cl}}
\def \im {\textup{im}}
\def \cchar {\textup{char}}
\def \coker {\textup{coker}}
\def \ker {\textup{ker}}
\def \Sel {\textup{Sel}}
\def \Selphi {\Sel^{(\phi)}}
\def \Selphih {\Sel^{(\phih)}}
\def \Selpsi {\Sel^{(\psi)}}
\def \Selpsih {\Sel^{(\psih)}}
\def \Seltwo {\Sel^{(2)}}
\def \Selthree {\Sel^{(3)}}


    \DeclareFontFamily{U}{wncy}{}
    \DeclareFontShape{U}{wncy}{m}{n}{<->wncyr10}{}
    \DeclareSymbolFont{mcy}{U}{wncy}{m}{n}
    \DeclareMathSymbol{\Sha}{\mathord}{mcy}{"58} 


==> IntegersImportThings.tex <==
\begin{comment}




\end{comment}
